Discovery and analysis of three magnetic hot subdwarf stars: evidence for merger-induced magnetic fields

Magnetic fields can play an important role in stellar evolution. Among white dwarfs, the most common stellar remnant, the fraction of magnetic systems is more than 20 per cent. The origin of magnetic fields in white dwarfs, which show strengths ranging from 40 kG to hundreds of MG, is still a topic of debate. In contrast, only one magnetic hot subdwarf star has been identified out of thousands of known systems. Hot subdwarfs are formed from binary interaction, a process often associated with the generation of magnetic fields, and will evolve to become white dwarfs, which makes the lack of detected magnetic hot subdwarfs a puzzling phenomenon. Here we report the discovery of three new magnetic hot subdwarfs with field strengths in the range 300-500 kG. Like the only previously known system, they are all helium-rich O-type stars (He-sdOs). We analysed multiple archival spectra of the three systems and derived their stellar properties. We find that they all lack radial velocity variability, suggesting formation via a merger channel. However, we derive higher than typical hydrogen abundances for their spectral type, which are in disagreement with current model predictions. Our findings suggest a lower limit to the magnetic fraction of hot subdwarfs of 0.147 (+0.143/-0.047) per cent, and provide evidence for merger-induced magnetic fields which could explain white dwarfs with field strengths of 50-150 MG, assuming magnetic flux conservation.

==> mag_sd_table.tex <==
%\documentclass{standalone}
%\usepackage{amsmath,txfonts,color}
%\usepackage{natbib}
%\usepackage[colorlinks=true,urlcolor=black]{hyperref}
%\begin{document}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lrrrrrrr}
\hline\hline
Star & Sp. Type & RVV & ref & T$_{\rm eff}$ (K) &$\log$ g &$\log$ y & ref  \\
\hline
%Name                      SpClass      RVV    ref     Teff  eTeff  logg elogg logy   elogy  Ref                
SB290               & sdB+K   &  ?    &   G    & 26300$\pm\phantom{0}$100 &  5.31$\pm$0.01 &$-$2.52$\pm$0.08 & 1 \\ %\citep{2013A&A...557A.122G}\\             
HD 4539             & sdB     &  no   &   S,K,E& 23200$\pm\phantom{0}$100 &  5.20$\pm$0.01 &$-$2.27$\pm$0.24 &  2\\ %\citep{2018A&A...618A..86S}\\
PHL 932             & sdB     &  no   &   K,E  & 33644$\pm\phantom{0}$500 &  5.74$\pm$0.05 &$-$1.64$\pm$0.05 &  3\\ %\citep{2005A&A...430..223L}\\
PG0133+114          & sdB+WD  &  yes  &   E    & 30073$\pm\phantom{0}$201 &  5.70$\pm$0.04 &$-$2.14$\pm$0.04 & 4\\ %\citep{2021ApJS..256...28L}\\
SB707               & sdB+WD  &  yes  &   E    & 35400$\pm\phantom{0}$500 &  5.90$\pm$0.05 &$-$2.90$\pm$0.10 & 5\\ %\citep{2006A&A...452..579O}\\
PG0342+026          & sdB     &  no   &   E,S  & 26000$\pm$1100           &  5.59$\pm$0.12 &$-$2.69$\pm$0.10 & 1 \\ %\citep{2013A&A...557A.122G}\\
HD76431             & sdB     &  no   & R,Kh,E & 31180$\pm\phantom{0}$220 &  4.67$\pm$0.03 &$-$1.58$\pm$0.05 &  6\\ %\citep{2014MNRAS.445.4086K}\\
HD127493            & He-sdO  &  no   &   E    & 42070$\pm\phantom{0}$180 &  5.61$\pm$0.04 &$+$0.33$\pm$0.06 &  7\\ %\citep{2019A&A...630A.130D}\\
HD149382            & sdB     &  no   &   J    & 34200$\pm\phantom{0}$1000&  5.89$\pm$0.15 &$-1$.60$\pm$0.10 &  8\\ %\citep{1994ApJ...432..351S}\\ 
HD171858            & sdB+WD  &  yes  &   E    & 27200$\pm\phantom{0}$800 &  5.30$\pm$0.10 &$-$2.84$\pm$0.10 & 9 \\ %\citep{2010A&A...519A..25G}\\
HD188112            & sdB+WD  &  yes  &   H    & 21500$\pm\phantom{0}$500 &  5.66$\pm$0.06 &$-$5.00          & 10 \\ %\citep{2003A&A...411L.477H}\\
HD205805            & sdB     &  no   &   E    & 25000$\pm\phantom{0}$500 &  5.00$\pm$0.10 &$-$2.00$\pm$0.20 & 11 \\ %\citep{2006BaltA..15..107P}\\
JL87                & He-sdB  &  no   &   E    & 25800$\pm$1000           &  4.8$\pm$0.30  &$+$0.33          & 12 \\ %\citep{2007A&A...465..541A}\\
SB 815              & sdB     &  no   &   K    & 27200$\pm\phantom{0}$550 &  5.39$\pm$0.10 &$-$2.94$\pm$0.01 & 2 \\ %\citep{2018A&A...618A..86S}\\
CW 83 0512$-$08     & sdOB    &  no   &   E,S  & 38400$\pm$1100           &  5.70$\pm$0.12 &$-$0.73$\pm$ 0.10& 1  \\ %\citep{2013A&A...557A.122G}\\
CPD-64$^\circ$481   & sdB+BD? &  yes  &   E    & 27500$\pm\phantom{0}$500 &  5.60$\pm$0.05 &$-$2.50$\pm$0.10 & 5 \\ %\citep{2006A&A...452..579O}\\           
CD-31$^\circ$4800   & He-sdO  &  no   &   E    & 42230$\pm\phantom{0}$300 &  5.60$\pm$0.10 &$+$2.61$\pm$0.20 & 13 \\ %\citep{2018A&A...620A..36S}\\
PG0909+276          & sdOB    &  no   &   E   & 35500$\pm\phantom{0}$500  &  6.09$\pm$0.05 &$-$1.00$\pm$0.10 & 1 \\ %\citep{2013A&A...557A.122G}\\
LSIV-14$^\circ$116  & He-sdO  &  no   &   JS   & 35150$\pm\phantom{0}$111 &  5.88$\pm$0.02 &$-$0.62$\pm$0.01 & 14 \\ %\citep{2015A&A...576A..65R}\\       
SB 410              & sdB+WD  &  yes  &   E    & 27600$\pm\phantom{0}$500 &  5.43$\pm$0.05 &$-$2.71$\pm$0.10 &  9 \\ %\citep{2010A&A...519A..25G}\\           
SB459               & sdB     &       &        & 24900$\pm\phantom{0}$500 &  5.35$\pm$0.10 &$-$2.58$\pm$0.10 & 15 \\ %\citep{2020MNRAS.495.2844S}\\   
LB1516              & sdB+WD  &  yes  &   E    & 25200$\pm$1100           &  5.41$\pm$0.12 &$-$2.78$\pm$0.10 &  1 \\ %\citep{2013A&A...557A.122G}\\
JL194               & sdB     &  no   &   E    & 25770$\pm\phantom{0}$380 &  5.21$\pm$0.06 &$-$2.69$\pm$0.06 & 16 \\ %\citep{2021A&A...651A.121U}\\
GD1110              & sdB+dM/BD &yes  &   E    & 26500$\pm$1100           &  5.38$\pm$0.12 &$-$2.54$\pm$0.10 & 1 \\ %\citep{2013A&A...557A.122G}\\
LSIV-12$^\circ$1    & sdO     &  no   &   E    & 60000$\pm$\phantom{0}5000&  4.50$\pm$0.50 &$-$0.95$\pm$0.20 & 17 \\ %\citep{1987Msngr..47...36H}\\            
LSE263              & He-sdO  &  no   &   K    & 72300$\pm$5380           &  5.49$\pm$0.11 &$+$0.02$\pm$2.10 & 18 \\ %\citep{2012MNRAS.427.2180N}\\
LSE153              & He-sdO  &       &        & 70000$\pm$1500           &  4.75$\pm$0.15 &                 & 19 \\ %\citep{1989A&A...222..150H}\\
BD+28$^\circ$4211   & sdO     &  no   &   L,H  & 81300$\pm$1200           &  6.52$\pm$0.05 &$-$1.12$\pm$0.05 & 20 \\ %\citep{2015A&A...579A..39L}\\
LSE21               & sdO     &       &        &                          &                &                 &   \\
GD687               & sdB+WD  &  yes  &   G    & 24350$\pm\phantom{0}$360 &  5.32$\pm$0.05 &$-$2.38          & 3 \\ %\citep{2005A&A...430..223L}\\
GD1669              & sdB     &    -  &        & 34126$\pm\phantom{0}$360 &  5.77$\pm$0.05 &$-$1.36          & 3 \\ %\citep{2005A&A...430..223L}\\
GD108               & sdB+x   &  yes  &   C    & 27760$\pm\phantom{0}$670 &  5.60$\pm$0.11 &$<-$3.0          & 21 \\ %\citep{2007ApJ...654..499K} \\
WD1153-484          & sdB     &       &        & 30080$\pm\phantom{0}$660 &  5.15$\pm$0.10 &$<-$3.0          &  21 \\ %\citep{2007ApJ...654..499K}\\
Balloon 090100001   & sdB     &  no   &   T    & 29446$\pm\phantom{0}$500 &  5.33$\pm$0.10 &$-$2.54$\pm$0.20 &  22 \\ %\citep{2004A&A...418..243O}\\
Feige34             & sdO     &       &        & 62550$\pm\phantom{0}$600 &  5.99$\pm$0.03 &$-$1.79$\pm$0.04 &  \\ %\citep{2018A&A...609A..89L}\\
Feige66             & sdB     &       &        & 33220$\pm\phantom{0}$370 &  6.14$\pm$0.08 &$-$1.61$\pm$0.11 & 23 \\ %\citep{2018ApJ...868...70L}\\
BD+75$^\circ$325    & sdO     &  no   &  s17   & 52000$\pm$2000           &  5.50$\pm$0.20 &$+$0.00          & 23 \\ %\citep{1997ApJ...485..843L}\\
\hline
\end{tabular}

comment: x=companion type unkown, RV curve not solved (Copperwheat+2011)

Magnetic field measurement (non-FORS)

 \citet{2006ApJ...648..559V}, %Feige 34: Valyavin 2006: 5kG (Landstreet et al. doubt it.)

 \citet{2013ARep...57..751S} %<~40G, Balloon 090100001 Savanow+2013:

\citet{2012ASPC..452...87P} %(ESPANDOS): <200G Feige 66: Petit et al. 

\citet{1996A&A...312L...5E} %: BD+75 325: Elkin 1996 1680+-60G dubious

RVV:

E: \citet{2005A&A...442.1023E} % Edelmann (2005) RVVs published, non-RVVs (priv. com.): unpublished supplement: 

S17: Schork 2017, teacher's thesis (FAU)

S:  \citet{2020arXiv200204545S} Silvotti+ 2020

J: \citet{2011AIPC.1331..304J} %Jacobs+ (2011) 

K: \citet{2015MNRAS.450.3514K} % K: Kawka+ (2015)

Kh:  \citet{2014MNRAS.445.4086K} %Khalack+ (2014)

R: \citet{2001A&A...379..235R} % Ramspeck+ 2001

L: \citet{2015A&A...579A..39L} %Latour+ 2015 

H: \citet{1999PASP..111.1144H}% Herbig 1999

JS: \citet{2015MNRAS.446.1889J} %Jeffery+, 2015 

C: \citet{2011MNRAS.415.1381C}  %Copperwheat+2011 

G:  \citet{2010A&A...515A..37G} % Geier+2010

T: \citet{2008 2008A&A...492..815T} % Telting+ 2008

%\end{tabular}
%\end{table}

\bibliographystyle{mnras}
\bibliography{table_apendix} %          
\end{document}

@ARTICLE{2011MNRAS.415.1381C,
       author = {{Copperwheat}, C.~M. and {Morales-Rueda}, L. and {Marsh}, T.~R. and {Maxted}, P.~F.~L. and {Heber}, U.},
        title = "{Radial-velocity measurements of subdwarf B stars}",
      journal = {\mnras},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = aug,
       volume = {415},
       number = {2},
        pages = {1381-1395},
          doi = {10.1111/j.1365-2966.2011.18786.x},
archivePrefix = {arXiv},
       eprint = {1103.4745},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.415.1381C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2005A&A...442.1023E,
       author = {{Edelmann}, H. and {Heber}, U. and {Altmann}, M. and {Karl}, C. and {Lisker}, T.},
        title = "{High resolution spectroscopy of bright subdwarf B stars. I. Radial velocity variables}",
      journal = {\aap},
     keywords = {stars: subdwarfs, stars: horizontal-branch, stars: fundamental parameters, binaries: close, Astrophysics},
         year = 2005,
        month = nov,
       volume = {442},
       number = {3},
        pages = {1023-1030},
          doi = {10.1051/0004-6361:20053267},
archivePrefix = {arXiv},
       eprint = {astro-ph/0507024},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...442.1023E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2011AIPC.1331..304J,
       author = {{Jacobs}, Valery A. and {{\O}stensen}, Roy H. and {van Winckel}, Hans and {Bloemen}, Steven and {P{\'a}pics}, Peter I. and {Raskin}, Gert and {Debosscher}, Jonas and {Uttenthaler}, Stefan and {van Aarle}, Els and {Waelkens}, Christoffel and {Bauwens}, Eva and {Verhoelst}, Tijl and {Gielen}, Clio and {Lehmann}, Holger and {Oreiro}, Raquel},
        title = "{HERMES High-Resolution Spectroscopy of HD 149382--Where Did the Planet Go?}",
     keywords = {spectroscopy, telescopes, stellar evolution, spectral analysis, 95.55.Qf, 95.55.-n, 97.60.Lf, 97.10.Ri, Photometric polarimetric and spectroscopic instrumentation, Astronomical and space-research instrumentation, Black holes, Luminosities, magnitudes, effective temperatures colors and spectral classification, Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Planetary Systems Beyond the Main Sequence},
         year = 2011,
       editor = {{Schuh}, Sonja and {Drechsel}, Horst and {Heber}, Ulrich},
       series = {American Institute of Physics Conference Series},
       volume = {1331},
        month = mar,
        pages = {304-309},
          doi = {10.1063/1.3556216},
archivePrefix = {arXiv},
       eprint = {1101.4158},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AIPC.1331..304J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020arXiv200204545S,
       author = {{Silvotti}, Roberto and {Ostensen}, Roy H. and {Telting}, John H.},
        title = "{No close companions to a sample of bright sdB stars}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = feb,
          eid = {arXiv:2002.04545},
        pages = {arXiv:2002.04545},
archivePrefix = {arXiv},
       eprint = {2002.04545},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200204545S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2005A&A...442.1023E,
       author = {{Edelmann}, H. and {Heber}, U. and {Altmann}, M. and {Karl}, C. and {Lisker}, T.},
        title = "{High resolution spectroscopy of bright subdwarf B stars. I. Radial velocity variables}",
      journal = {\aap},
     keywords = {stars: subdwarfs, stars: horizontal-branch, stars: fundamental parameters, binaries: close, Astrophysics},
         year = 2005,
        month = nov,
       volume = {442},
       number = {3},
        pages = {1023-1030},
          doi = {10.1051/0004-6361:20053267},
archivePrefix = {arXiv},
       eprint = {astro-ph/0507024},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...442.1023E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.445.4086K,
       author = {{Khalack}, V. and {Yameogo}, B. and {LeBlanc}, F. and {Fontaine}, G. and {Green}, E. and {Van Grootel}, V. and {Petit}, P.},
        title = "{Spectral analysis and abundances of the post-HB star HD 76431}",
      journal = {\mnras},
     keywords = {stars: abundances, stars: atmospheres - stars: chemically peculiar, stars: horizontal branch, stars: individual: HD 76431, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = dec,
       volume = {445},
       number = {4},
        pages = {4086-4093},
          doi = {10.1093/mnras/stu2012},
archivePrefix = {arXiv},
       eprint = {1409.7669},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.445.4086K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2015A&A...579A..39L,
       author = {{Latour}, M. and {Fontaine}, G. and {Green}, E.~M. and {Brassard}, P.},
        title = "{A non-LTE analysis of the hot subdwarf O star BD+28{\textdegree}4211. II. The optical spectrum}",
      journal = {\aap},
     keywords = {stars: atmospheres, stars: fundamental parameters, subdwarfs, stars: individual: BD+28{\textdegree}4211, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jul,
       volume = {579},
          eid = {A39},
        pages = {A39},
          doi = {10.1051/0004-6361/201525999},
archivePrefix = {arXiv},
       eprint = {1504.06417},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...579A..39L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999PASP..111.1144H,
       author = {{Herbig}, G.~H.},
        title = "{The Optical Spectrum of the O-Type Subdwarf BD +28 deg4211}",
      journal = {\pasp},
     keywords = {STARS: EARLY-TYPE, STARS: INDIVIDUAL: ALPHANUMERIC: BD +28 DEG4211},
         year = 1999,
        month = sep,
       volume = {111},
       number = {763},
        pages = {1144-1148},
          doi = {10.1086/316426},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999PASP..111.1144H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2015MNRAS.450.3514K,
       author = {{Kawka}, A. and {Vennes}, S. and {O'Toole}, S. and {N{\'e}meth}, P. and {Burton}, D. and {Kotze}, E. and {Buckley}, D.~A.~H.},
        title = "{New binaries among UV-selected, hot subdwarf stars and population properties}",
      journal = {\mnras},
     keywords = {binaries: close, binaries: spectroscopic, subdwarfs, white dwarfs, ultraviolet: stars, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jul,
       volume = {450},
       number = {4},
        pages = {3514-3548},
          doi = {10.1093/mnras/stv821},
archivePrefix = {arXiv},
       eprint = {1504.03241},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.3514K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2015MNRAS.446.1889J,
       author = {{Jeffery}, C.~S. and {Ahmad}, A. and {Naslim}, N. and {Kerzendorf}, W.},
        title = "{Radial-velocity measurements of the pulsating zirconium star: LS IV-14{\textdegree}116}",
      journal = {\mnras},
     keywords = {asteroseismology, stars: chemically peculiar, stars: individual (LS IV-14{\textdegree}116), subdwarf, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = jan,
       volume = {446},
       number = {2},
        pages = {1889-1894},
          doi = {10.1093/mnras/stu2203},
archivePrefix = {arXiv},
       eprint = {1410.5732},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.446.1889J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2005A&A...430..223L,
       author = {{Lisker}, T. and {Heber}, U. and {Napiwotzki}, R. and {Christlieb}, N. and {Han}, Z. and {Homeier}, D. and {Reimers}, D.},
        title = "{Hot subdwarfs from the ESO Supernova Ia Progenitor Survey.  I. Atmospheric parameters and cool companions of sdB stars}",
      journal = {\aap},
     keywords = {binaries: spectroscopic, stars: abundances, stars: atmospheres, stars: fundamental parameters, stars: horizontal-branch, subdwarfs, Astrophysics},
         year = 2005,
        month = jan,
       volume = {430},
        pages = {223-243},
          doi = {10.1051/0004-6361:20040232},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409136},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...430..223L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...654..499K,
       author = {{Kawka}, A. and {Vennes}, S. and {Schmidt}, G.~D. and {Wickramasinghe}, D.~T. and {Koch}, R.},
        title = "{Spectropolarimetric Survey of Hydrogen-rich White Dwarf Stars}",
      journal = {\apj},
     keywords = {Magnetic Fields, Stars: White Dwarfs, Astrophysics},
         year = 2007,
        month = jan,
       volume = {654},
       number = {1},
        pages = {499-520},
          doi = {10.1086/509072},
archivePrefix = {arXiv},
       eprint = {astro-ph/0609273},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...654..499K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2010A&A...515A..37G,
       author = {{Geier}, S. and {Heber}, U. and {Kupfer}, T. and {Napiwotzki}, R.},
        title = "{Binaries discovered by the SPY project . V. GD 687 - a massive double degenerate binary progenitor that will merge within a Hubble time}",
      journal = {\aap},
     keywords = {binaries: spectroscopic, subdwarfs, stars: individual:, GD 687, stars: rotation, supernovae: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = jun,
       volume = {515},
          eid = {A37},
        pages = {A37},
          doi = {10.1051/0004-6361/200912545},
archivePrefix = {arXiv},
       eprint = {1003.4113},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...515A..37G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ARep...57..751S,
       author = {{Savanov}, I.~S. and {Romaniuk}, I.~I. and {Semenko}, E.~A. and {Dmitrienko}, E.~S.},
        title = "{The presence of a magnetic field on the pulsating subdwarf Balloon 090100001. Observations of 2012}",
      journal = {Astronomy Reports},
         year = 2013,
        month = oct,
       volume = {57},
       number = {10},
        pages = {751-756},
          doi = {10.1134/S1063772913090059},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ARep...57..751S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2008A&A...492..815T,
       author = {{Telting}, J.~H. and {Geier}, S. and {{\O}stensen}, R.~H. and {Heber}, U. and {Glowienka}, L. and {Nielsen}, T. and {Oreiro}, R. and {Frandsen}, S.},
        title = "{Time-resolved high-resolution spectroscopy of the bright pulsating subdwarf B star Balloon 090100001}",
      journal = {\aap},
     keywords = {stars: subdwarfs, line: profiles, stars: early-type, stars: oscillations, stars: variables: general, stars: individual: Balloon 090100001},
         year = 2008,
        month = dec,
       volume = {492},
       number = {3},
        pages = {815-821},
          doi = {10.1051/0004-6361:200810759},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...492..815T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004A&A...418..243O,
       author = {{Oreiro}, R. and {Ulla}, A. and {P{\'e}rez Hern{\'a}ndez}, F. and {{\O}stensen}, R. and {Rodr{\'\i}guez L{\'o}pez}, C. and {MacDonald}, J.},
        title = "{<ASTROBJ>Balloon 090100001</ASTROBJ>: A bright, high amplitude sdB pulsator}",
      journal = {\aap},
     keywords = {stars: early-type, stars: subdwarfs, stars: oscillations, stars: individual: Balloon 090100001},
         year = 2004,
        month = apr,
       volume = {418},
        pages = {243-247},
          doi = {10.1051/0004-6361:20035844},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...418..243O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJ...648..559V,
       author = {{Valyavin}, G. and {Bagnulo}, S. and {Fabrika}, S. and {Reisenegger}, A. and {Wade}, G.~A. and {Han}, Inwoo and {Monin}, D.},
        title = "{A Search for Kilogauss Magnetic Fields in White Dwarfs and Hot Subdwarf Stars}",
      journal = {\apj},
     keywords = {stars: individual (WD 1036+433), stars: individual (WD 1647+591), stars: individual (WD 1105-048), Stars: Magnetic Fields, Stars: White Dwarfs, Astrophysics},
         year = 2006,
        month = sep,
       volume = {648},
       number = {1},
        pages = {559-564},
          doi = {10.1086/505781},
archivePrefix = {arXiv},
       eprint = {astro-ph/0605401},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...648..559V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2018A&A...609A..89L,
       author = {{Latour}, M. and {Chayer}, P. and {Green}, E.~M. and {Irrgang}, A. and {Fontaine}, G.},
        title = "{Spectral analysis of four surprisingly similar hot hydrogen-rich subdwarf O stars}",
      journal = {\aap},
     keywords = {stars: atmospheres, stars: abundances, subdwarfs, stars: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = jan,
       volume = {609},
          eid = {A89},
        pages = {A89},
          doi = {10.1051/0004-6361/201731496},
archivePrefix = {arXiv},
       eprint = {1710.06716},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...609A..89L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...868...70L,
       author = {{Lei}, Zhenxin and {Zhao}, Jingkun and {N{\'e}meth}, P{\'e}ter and {Zhao}, Gang},
        title = "{New Hot Subdwarf Stars Identified in Gaia DR2 with LAMOST DR5 Spectra}",
      journal = {\apj},
     keywords = {Hertzsprung{\textendash}Russell and C{\textendash}M diagrams, subdwarfs, surveys, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = nov,
       volume = {868},
       number = {1},
          eid = {70},
        pages = {70},
          doi = {10.3847/1538-4357/aae82b},
archivePrefix = {arXiv},
       eprint = {1810.09625},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...868...70L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{1997ApJ...485..843L,
       author = {{Lanz}, Thierry and {Hubeny}, Ivan and {Heap}, Sara R.},
        title = "{Non-LTE Line-blanketed Model Atmospheres of Hot Stars. III. Hot Subdwarfs: The sdO Star BD +75{\textdegree}325}",
      journal = {\apj},
     keywords = {Stars: Abundances, Stars: Atmospheres, Stars: Early-Type, Stars: Fundamental Parameters, Stars: Individual: Alphanumeric: BD +75{\textdegree}325, stars: mass-loss},
         year = 1997,
        month = aug,
       volume = {485},
       number = {2},
        pages = {843-858},
          doi = {10.1086/304455},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...485..843L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2012ASPC..452...87P,
       author = {{Petit}, P. and {Van Grootel}, V. and {Bagnulo}, S. and {Charpinet}, S. and {Wade}, G.~A. and {Green}, E.~M.},
        title = "{High-resolution Spectropolarimetric Observations of Hot Subdwarfs}",
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
    booktitle = {Fifth Meeting on Hot Subdwarf Stars and Related Objects},
         year = 2012,
       editor = {{Kilkenny}, D. and {Jeffery}, C.~S. and {Koen}, C.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {452},
        month = mar,
        pages = {87},
archivePrefix = {arXiv},
       eprint = {1110.5227},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ASPC..452...87P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996A&A...312L...5E,
       author = {{Elkin}, V.~G.},
        title = "{Magnetic fields in hot subdwarfs.}",
      journal = {\aap},
     keywords = {STELLAR SPECTROSCOPY, STARS: HOT SUBDWARFS, STARS: INDIVIDUAL BD+75 325, BD+25 2534, STARS: MAGNETIC FIELDS},
         year = 1996,
        month = aug,
       volume = {312},
        pages = {L5-L8},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&A...312L...5E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


